UniDM: A Unified Framework for Data Manipulation with Large Language Models

Designing effective data manipulation methods is a long standing problem in data lakes. Traditional methods, which rely on rules or machine learning models, require extensive human efforts on training data collection and tuning models. Recent methods apply Large Language Models (LLMs) to resolve multiple data manipulation tasks. They exhibit bright benefits in terms of performance but still require customized designs to fit each specific task. This is very costly and can not catch up with the requirements of big data lake platforms. In this paper, inspired by the cross-task generality of LLMs on NLP tasks, we pave the first step to design an automatic and general solution to tackle with data manipulation tasks. We propose UniDM, a unified framework which establishes a new paradigm to process data manipulation tasks using LLMs. UniDM formalizes a number of data manipulation tasks in a unified form and abstracts three main general steps to solve each task. We develop an automatic context retrieval to allow the LLMs to retrieve data from data lakes, potentially containing evidence and factual information. For each step, we design effective prompts to guide LLMs to produce high quality results. By our comprehensive evaluation on a variety of benchmarks, our UniDM exhibits great generality and state-of-the-art performance on a wide variety of data manipulation tasks.

==> sec-discussion.tex <==
\section{Future Research Directions}
\label{sec:discussion}

Although we have made some progress on applying LLMs to data manipulation tasks on data lakes, there still reserves much room for improvement upon our work. In this section, we summarize some future research directions in terms of different perspectives of data, model, algorithm and efficiency as follows.

\sstitle{Integration with Domain Knowledge}
From the evaluation results in Section~\ref{sec:exp-2}, we observe that \sys can perform well on universal data but may fall on domain specific data. However, data lakes often contain data from highly specialized domains, e.g., financial, biological and academic data. Therefore, it is worthwhile to investigate how to incorporate domain-specific knowledge into the knowledge base of LLMs. Currently, the widely adopted method is to fine-tune the LLMs with domain specific data. Whereas, there still remain some challenges for fine-tuning. First is how to extract high quality data from data lakes as a corpus to tune the LLMs. The second is how to design fine-tuning methods for LLMs which are not open-source (such as GPT-3~\cite{brown2020language}). Besides, it is very interesting to explore new integration methods except fine-tuning LLMs.

\sstitle{Extension to More Data Types}
Our solution on data manipulation tasks mainly considers the structured data in relation tables in this paper. We present an example in Section~\ref{sec:exp} on applying our method to retrieve information on semi-structured data (e.g., HTML data). However, data lake contains various data including semi-structured (e.g., xml), unstructured (e.g., graph) data and even multi-modal data (e.g., tables, texts and images). It is very helpful to extend our methods to process these types of data. 

\sstitle{Designing Large Models for DB Tasks}
Currently, the LLMs are mainly trained on a corpus of texts to resolve NLP tasks. Although we could design serialization functions and prompts to apply LLMs on tabular data, it is essentially a process of cutting the foot to fit the shoe. A better way is to design and train large models on tabular (and other types of) data from scratch to capture semantics for database tasks. This is a very challenging but promising direction. Some previous works have attempted to leverage BERT (e.g., TaBERT \cite{yin2020tabert}, TaPas \cite{herzig2020tapas}, TaPEx \cite{liu2021tapex}, Tableformer \cite{yang2022tableformer}, TURL\cite{deng2022turl}) to understand (semi-)structured data. However, all of the concepts, model structures, training methods and the whole paradigm of large models need to be re-designed to fit database tasks.

\sstitle{Efficiency Consideration}
LLMs applied in our method bring benefits in terms of the result accuracy but also entail a significant increase in computational resource and memory cost. Our \sys requires more GPU resources to do inference on LLMs than conventional methods. Therefore, in the future work, it is rather important to consider how to improve the efficiency while retaining the effectiveness of LLM-based methods. We suggest two possible ways. One is to design more efficient retrieval methods to extract very relevant information from data to minimize the computation overhead. Another way is to adapt to select the LLMs with minimal computation cost to fulfill each task. As we show in Table~\ref{tab:ft}, a fine-tuned LLM in a smaller size is possible to match the performance of a universal LLM in a much larger size. 

\sstitle{LLM-based and Traditional Methods}
In spite of our LLM-based solutions exhibiting superiority in terms of result effectiveness, they can not totally replace traditional methods. Until now, LLM is still a black-box which is difficult to interpret, debug and analyze. These are all risky factors for database systems which require rock-solid stability. Traditional methods relying on rules and logic tuned by human experience over decades have their unique advantages. They are more friendly to system deployment. Therefore, LLM-based and traditional methods are not conflicting but rather complementary to each other. It would be very practical to combine their advantages together to control the deployment risk while still attaining high result effectiveness.

\sstitle{Limitations of \sys}
\sys can benefit from explicitly retrieving data, potentially containing evidence and factual information, before the processing of data manipulation. However, the model may be unreliable when dealing with domain-specific knowledge that is required for commercial use cases. In such scenarios, LLMs can generate information that may be problematic in practical applications where factual accuracy is crucial. Another limitation is explainability. In most data applications (e.g., root cause analysis), a good explanation that includes all the rules applied to reach a conclusion can be valuable to the user. While LLMs have exhibited remarkable success in various data tasks, their ability to reason and explain is often viewed as a limitation. Our method here does not address this class of problem and likely prompt engineering would be required to solve it.


